Learning and generalization of one-hidden-layer neural networks, going beyond standard Gaussian data

This paper analyzes the convergence and generalization of training a one-hidden-layer neural network when the input features follow the Gaussian mixture model consisting of a finite number of Gaussian distributions. Assuming the labels are generated from a teacher model with an unknown ground truth weight, the learning problem is to estimate the underlying teacher model by minimizing a non-convex risk function over a student neural network. With a finite number of training samples, referred to the sample complexity, the iterations are proved to converge linearly to a critical point with guaranteed generalization error. In addition, for the first time, this paper characterizes the impact of the input distributions on the sample complexity and the learning rate.

==> CISS_mixed_Gaussian (1)/Algorithm.tex <==
\section{Algorithm}
We propose a gradient descent algorithm with tensor initialization method to solve \eqref{eqn:problem}. The method starts from an initialization $\bfW_0 \in \R^{d\times K}$ computed from the tensor initialization method (Subroutine \ref{TensorInitialization}) and then updates the iteration $\bfW_t$ using gradient descent   with the step size $\eta_0$. The pseudo-code is summarized in Algorithm \ref{gd}.



The tensor initialization algorithm is summarized in Subroutine \ref{TensorInitialization}. While existing tensor decomposition methods in \cite{JSA14} and \cite{ZSJB17} only apply for standard Gaussian distribution, we extend the methods to Gaussian mixture models. The intuition is similar to that in \cite{ZSJB17}, where the directions of $\{\bfw_j^*\}_{j\in[K]}$ are first estimated through decomposing the high-order tensor, and then the corresponding magnitudes are estimated through solving a linear regression problem. However, the high-order tensors are defined in a fairly different way because of the difference between input distributions. Formally, the high order tensor $\bfQ_j$'s are defined in Definition \ref{def: M}.
\begin{definition}\label{def: M}
 For $j=1,2,3$, we define 
\begin{equation}\label{eqn:mj}
    \bfQ_j:=\mathbb{E}_{\bfx\sim\sum_{l=1}^L\lambda_l\mathcal{N}(\bfmu_l,\bfSg_l)}[y\cdot (-1)^j p^{-1}(\bfx)\nabla^{(j)}p(\bfx)], 
 %   \bfM_j:=\mathbb{E}_{\bfx\sim\sum_{l=1}^L\lambda_l\mathcal{N}(\bfmu_l,\sigma_l^2\bfI)}[y\cdot (-1)^j\frac{\nabla^{(m)}p(\bfx)}{p(\bfx)}],\ j=1,2,3  
\end{equation}
where $p(\bfx)$ is
\begin{equation}\label{eqn:p}
 p(\boldsymbol{x})=\sum_{l=1}^L\lambda_l(2\pi)^{-\frac{d}{2}}\exp\big(-\frac{1}{2}(\boldsymbol{x}-\boldsymbol{\mu}_l)^\top(\boldsymbol{x}-\boldsymbol{\mu}_l)\big).
 \end{equation}
\end{definition}

\begin{algorithm}
\caption{Gradient Descent with Tensor Initialization}\label{gd}
\begin{algorithmic}[1]
\STATE{\textbf{Input: }} 
 Training data $\{(\bfx_i,y_i)\}_{i=1}^n$, the step size $\eta_0= \big( \sum_{l=1}^L\lambda_l (\|{\bfmu}_l\|_\infty+1)^2 \big)^{-1}$;
\STATE{\textbf{Initialization: }}$\bfW_{0}\leftarrow$ Tensor initialization method via Subroutine \ref{TensorInitialization};
\FOR{$t=0,1,\cdots,T-1$}
\item $\bfW_{t+1}= \bfW_t-\eta_0\nabla f_n(\bfW)$
\ENDFOR
\STATE{\textbf{Output: }} $\bfW_T$
\end{algorithmic}
\end{algorithm}

\floatname{algorithm}{Subroutine}
\setcounter{algorithm}{0}
\begin{algorithm}
\caption{Tensor Initialization Method}\label{TensorInitialization}
\begin{algorithmic}[1]
\STATE{\textbf{Input: }} Partition $\{(\bfx_i,y_i)\}_{i=1}^n$ into three disjoint subsets $\mathcal{D}_1$, $\mathcal{D}_2$, $\mathcal{D}_3$;
% \IF{the Gaussian Mixture distribution is not symmetric}
% \STATE Compute $\widehat{\bfQ}_2$ using $\mathcal{D}_1$. Estimate the subspace $\widehat{\bfU}$   by orthogonalizing the eigenvectors with respect to the $K$ largest eigenvalues of  $\widehat{\bfQ}_2$
% \ELSE \STATE Pick an arbitrary vector  $\boldsymbol{\alpha} \in \R^{d}$, and use $\mathcal{D}_1$ to compute $\widehat{\bfQ}_3(\bfI_d,\bfI_d,\boldsymbol{\alpha})$.  Estimate   $\widehat{\bfU}$   by orthogonalizing the eigenvectors with respect to the $K$ largest eigenvalues of   $\widehat{\bfQ}_3(\bfI_d,\bfI_d,\boldsymbol{\alpha})$.
% \ENDIF 
\STATE Compute $\widehat{\bfQ}_2$ using $\mathcal{D}_1$. Estimate the subspace $\widehat{\bfU}$  with respect to the largest $K$ eigenvectors of $\widehat{\bfQ}_2$;
\STATE Compute $\widehat{\bfR}_3=\widehat{\bfQ}_3(\widehat{\bfU},\widehat{\bfU},\widehat{\bfU})$ from data set $\mathcal{D}_2$. Obtain $\{\hat{\bfv}_i\}_{i\in[K]}$ by decomposing $\widehat{R}_3$;
\STATE $\boldsymbol{\bar{w}}_i^* = \widehat{\bfU}\hat{\bfv}_i$ for $i\in[K]$;
\STATE Compute $\widehat{\bfQ}_1$ from data set $\mathcal{D}_3$. Estimate the magnitude $\widehat{\bfz}$ by solving the optimization problem
    $$\widehat{\boldsymbol{z}}= \arg\min_{\boldsymbol{\alpha}\in\mathbb{R}^K}\frac{1}{2}\|\widehat{\bfQ}_1-\sum_{j=1}^K \alpha_j\boldsymbol{\bar{w}}_j^*\|^2;$$
\STATE \textbf{Return:} $\hat{z}_j\widehat{\bfU}\hat{\bfv}_j$ as the $j$th column of $\bfW_0$,  $j\in [K]$.
\end{algorithmic}
\end{algorithm}
Subroutine \ref{TensorInitialization} estimates the direction and magnitude of $\bfw_j^*, j\in[K]$ separately. The direction vector is defined as $\boldsymbol{\bar{w}}_j^*:=\bfw_j^*/\|\bfw_j^*\|$, and the corresponding magnitude $\|\bfw_j^*\|$ is denoted as $z_j$.
Line 2 estimates  the subspace  $\widehat{\bfU}$ spanned by $\{\bfw_1^*,\cdots,\bfw_K^*\}$ using $\widehat{\bfQ}_2$.  Lines 3-4 estimate the  direction vector $\boldsymbol{\bar{w}}_j^*$ by employing the KCL algorithm \cite{KCL15}. Line 5 estimates  the magnitude $z_j$. Finally, the returned estimation of $\bfW^*$ is calculated as $\hat{z}_j\widehat{\bfU}\hat{\bfv}_j$.

==> CISS_mixed_Gaussian (1)/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> CISS_mixed_Gaussian (1)/introduction.tex <==
\section{Introduction}
The recent success of machine learning mainly benefits from the developments of neural networks. It is surprising to witness the superior empirical performance in various applications ranging from imaging processing \cite{KSH12,HZRS16, KCKJ22} to natural language processing \cite{GMH13}. However, the lack of theoretical generalization guarantee has become a rising concern with the widespread utilization of neural networks. That is,  the learned model from a finite number of training samples has guaranteed test error on the unseen data. From the perspective of optimization, achieving guaranteed generalization is to obtain both a small training error and a bounded generalization gap (difference between the training and test errors), which are referred to convergence and generalization analysis. Despite the high test accuracy in numerical experiments, the convergence and generalization analysis are limited, and significant breakthroughs focus on shallow neural networks \cite{MMN18,JGH18,ZSJB17}. Nevertheless, it is well-known that training a one-hidden-layer neural network with only three nodes is NP-hard \cite{BR92}, and various assumptions are imposed to ensure feasible analysis.


One representative line of works studies the overparameterized neural networks, where the number of trainable parameters is far larger than the number of training samples. In particular, the optimization problem of training on overparameterized networks has no spurious local minima \cite{LSS14,LY17,ZBHRV16,SJL18}, and thus the random initialization can achieve bounded training errors. However, such learned models may suffer from over-fitting and cannot provide a generalization guarantee without additional assumptions. With the assumptions of infinite width of neurons, training a neural network via gradient descent can be approximated by a differential equation from the Mean Field (MF) view \cite{CB18b,MMN18,FGZZ19,Nguyen2019} or a Gaussian kernel processing from the Neural Tangent Kernel (NTK) view \cite{JGH18,ALS19,DZPS19,ZCZG20,ZG19, LWLC22}. In particular,  for one-hidden-layer neural networks,  \cite{MMM19,WLLM18,ALL19,ADHL19}
provide bounded generalization errors for some target functions with nice properties, i.e., even or infinitely smooth functions. Nevertheless, both MF and NTK frameworks require a significantly larger number of neurons  than that in practical cases.

For training neural networks with a fixed number of neurons, the landscapes of the objective functions are highly non-convex. They can contain intractably  many spurious local minima \cite{SS17} with multiple neurons.
This line of work follows the ``teacher-student'' setup, where the training data is generated by a teacher neural network. The learning is performed on a student network by minimizing the empirical risk functions of the training data.   
To achieve the optimal with guaranteed generalization, most of the theoretical works  with a fixed number of neurons assume the input belongs to standard Gaussian distributions (zero mean and unit variance) for feasible analysis \cite{ZSJB17,ZWXL20,ZWLC20_1,ZWLC20_2,ZWLC21,FCL20} with a few exceptions \cite{DLT18,MBM16}.
Nevertheless, the neural network considered in \cite{DLT18,MBM16} only contains a single neuron in the hidden layer, and the objective function has a large benign landscape near the desired point such that random initialization succeeds with constant probability regardless of the non-convexity. 
Other works considering non-Gaussian input features either require an infinitely large number of neurons \cite{MMN18,LL18} or cannot provide bounded generalization analysis \cite{YO19,GMKZ19,GRMK20,MKUZ20,GMMM20}. 

Overall, the generalization analysis of neural networks beyond the standard Gaussian input is  less investigated and has not received enough attention. On the one hand, Gaussian mixture models are widely employed in plenty of applications, including data clustering \cite{D99, FJ02, J10}, image segmentation \cite{PFJ06}, and few-shot learning \cite{YLX21}. 
On the other hand, 
the study of Gaussian mixture models casts an insight into understanding how the mean and variance of the input features affect the performance. In practice, the input distribution will affect the learning performance, and several data pre-processing techniques such as data whitened \cite{LBOM98} and batch normalization \cite{IS15} have been applied to accelerate the convergence rate and improve the generalization error.
Although various works \cite{BGSW18,CPM20,STIM18} have studied the enormous success of batch normalization from different scopes and provided different explanations,  none of them have studied from the perspective of generalization analysis. 
% the learning performance clearly depends on the input data distribution. \cite{LBOM98} states that the learning method converges faster if the inputs are whitened to be the standard Gaussian. Batch normalization \cite{IS15} modifies the mean and variance in each layer   and is a popular practical method to achieve fast and stable convergence. 

% The parameters of the mixture model can be estimated from data  by   the EM algorithm \cite{RW84} or the moment-based method \cite{HK13}, with theoretical performance guarantees, see, e.g., \cite{HN16,HDKW20,DHKJ20,DHKw20}.
\textbf{Contributions:} This paper provides a  theoretical analysis of learning one-hidden-layer neural networks when the input distribution   follows a Gaussian mixture model containing an arbitrary number of Gaussian distributions with arbitrary mean. Specific contributions include: 

1. \textbf{Proposition of a gradient descent algorithm and tensor initialization with Gaussian mixture inputs:} This is the first paper to propose a gradient descent with tensor initialization method for Gaussian mixture inputs.

2. \textbf{Guaranteed generalization error with Gaussian mixture inputs for binary classification problems:} For the first time, we give a guaranteed generalization error for binary classification problems when the inputs follow Gaussian mixture model.

3. \textbf{First sample complexity analysis depending on the parameters of the input distribution:} Our theorem provides the first explicit characterization of the required number of samples to learn the neural network. 
% The proposed algorithm enjoys a linear convergence rate, and the returned critical point are proved to approach the teacher model  in the order of $\sqrt{d\log{n}/n}$, where $d$ is the dimension of the feature, and $n$ is the number of samples. 

% We also characterize  the required number of samples for accurate estimation, referred to as the sample complexity, 
% as a function of  $d$, the number of neurons $K$, and the input distribution.  Our explicit bounds imply (1)  when the absolute value of any mean   in the Gaussian mixture model increases from zero, the sample complexity increases, and the algorithm converges slower, indicating that it will be more challenging to learn a model with a small test error; (2) The same phenomenon happens when any variance in the mixture model increases to infinity from a certain positive value, or if all the variances in the mixture model   approach  zero. Our results indicate that the training converges faster and requires fewer samples if the input data are zero mean with a certain non-zero variance. This can be viewed as one theoretical explanation in one-hidden-layer for the success of Batch normalization.  Moreover, to the best of our knowledge, \textit{this paper provides the first theoretical and explicit characterization about how the mean and variance of the  input distribution affect  the sample complexity and learning rate}. 

\textbf{Notations}: Vectors are in bold lowercase, and matrices and tensors
are in bold uppercase. Scalars are in normal fonts. Sets are in calligraphic fonts. For example, $\bfZ$ is a matrix, and $\bfz$ is a vector. $\mathcal{Z}$ is a set. $z_i$ denotes the $i$-th entry of $\bfz$, and $Z_{i,j}$ denotes the $(i,j)$-th entry of $\bfZ$. 
$[K]$ ($K>0$) denotes the set including integers from $1$ to $K$. $\bfI_d\in\mathbb{R}^{d\times d}$ and $\bfe_i$ represent the identity matrix in $\mathbb{R}^{d \times d}$ and the $i$-th standard basis vector, respectively. 
We use $\delta_i(\bfZ)$ to denote the $i$-th largest singular value of $\bfZ$. The matrix norm is defined as $\|\bfZ\|=\delta_1(\bfZ)$. The gradient and the Hessian of a function $f(\bfW)$ are  denoted by $\nabla f(\bfW)$ and $\nabla^2 f(\bfW)$, respectively.\\ %The outer product of  vectors $\bfz_i\in\mathbb{R}^{n_i}$, $i\in[l]$, is defined as $\bfT=\bfz_1\otimes \cdots\times \bfz_l\in\mathbb{R}^{n_1\times\cdots\times n_l}$ with $\bfT_{j_1\cdots j_l}=(\bfz_1)_{j_1}\cdots(\bfz_l)_{j_l}$.\\
Given a tensor $\bfT\in\mathbb{R}^{n_1\times n_2\times n_3}$ and   matrices $\bfA\in\mathbb{R}^{n_1\times d_1}$, $\bfB\in\mathbb{R}^{n_2\times d_2}$, $\bfC\in\mathbb{R}^{n_3\times d_3}$, the $(i_1,i_2, i_3)$-th entry of the tensor $\bfT(\bfA,\bfB, \bfC)$ is given by
\begin{equation}
    \sum_{i_1'}^{n_1}\sum_{i_2'}^{n_2}\sum_{i_3'}^{n_3}\bfT_{i_1',i_2', i_3'}{\bfA}_{i_1',i_1}{\bfB}_{i_2',i_2}{\bfC}_{i_3',i_3}.\label{T(A,B,C)}
\end{equation}
We follow the convention that $f(x)=O(g(x))$ (or $\Omega(g(x))$, $\Theta(g(x)))$ means that $f(x)$ is at most, at least, or in the order of $g(x)$, respectively. 

==> CISS_mixed_Gaussian (1)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{algorithm}
%\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{subfigure}

\newtheorem{lemma}{Lemma}
\newtheorem{thm}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}

\newtheorem{assumption}{Assumption}
\newtheorem{property}{Property}
\def\bfzero{{\boldsymbol{0}}}
\def\bfone{{{\bf1}}}
\def\bfa{{\boldsymbol a}}
\def\bfb{{\boldsymbol b}}
\def\bfc{{\boldsymbol c}}
\def\bfd{{\boldsymbol d}}
\def\bfe{{\boldsymbol e}}
\def\bff{{\boldsymbol f}}
\def\bfg{{\boldsymbol g}}
\def\bfh{{\boldsymbol h}}
\def\bfi{{\boldsymbol i}}
\def\bfj{{\boldsymbol j}}
\def\bfk{{\boldsymbol k}}
\def\bfl{{\boldsymbol l}}
\def\bfm{{\boldsymbol m}}
\def\bfn{{\boldsymbol n}}
\def\bfo{{\boldsymbol o}}
\def\bfp{{\boldsymbol p}}
\def\bfq{{\boldsymbol q}}
\def\bfr{{\boldsymbol r}}
\def\bfs{{\boldsymbol s}}
\def\bft{{\boldsymbol t}}
\def\bfu{{\boldsymbol u}}
\def\bfv{{\boldsymbol v}}
\def\bfw{{\boldsymbol w}}
\def\bfx{{\boldsymbol x}}
\def\bfy{{\boldsymbol y}}
\def\bfz{{\boldsymbol z}}
\def\bfmu{{\boldsymbol \mu}}
\def\bfsg{{\boldsymbol\sigma}}
\def\bfSg{{\boldsymbol\Sigma}}
\def\bfDT{{\boldsymbol\Delta}}
\def\bfLM{{\boldsymbol\Lambda}}

\def\bfA{{\boldsymbol A}}
\def\bfB{{\boldsymbol B}}
\def\bfC{{\boldsymbol C}}
\def\bfD{{\boldsymbol D}}
\def\bfE{{\boldsymbol E}}
\def\bfF{{\boldsymbol F}}
\def\bfG{{\boldsymbol G}}
\def\bfH{{\boldsymbol H}}
\def\bfI{{\boldsymbol I}}
\def\bfJ{{\boldsymbol J}}
\def\bfK{{\boldsymbol K}}
\def\bfL{{\boldsymbol L}}
\def\bfM{{\boldsymbol M}}
\def\bfN{{\boldsymbol N}}
\def\bfO{{\boldsymbol O}}
\def\bfP{{\boldsymbol P}}
\def\bfQ{{\boldsymbol Q}}
\def\bfR{{\boldsymbol R}}
\def\bfS{{\boldsymbol S}}
\def\bfT{{\boldsymbol T}}
\def\bfU{{\boldsymbol U}}
\def\bfV{{\boldsymbol V}}
\def\bfW{{\boldsymbol W}}
\def\bfX{{\boldsymbol X}}
\def\bfY{{\boldsymbol Y}}
\def\bfZ{{\boldsymbol Z}}
 
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\tcr}{\textcolor{red}}

\DeclareMathOperator\erf{erf}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{(\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

==> CISS_mixed_Gaussian (1)/problem.tex <==
\section{Problem Formulation}
In this paper, we consider the distribution $(\mathcal{X}, \mathcal{Y})$ over $(\bfx, y)\in \mathbb{R}^{d}\times \{+1, -1\}$, where $\mathcal{X}$ is the Gaussian mixture distribution \cite{P94, TSM85, HK13} such that 
\begin{equation}
\bfx \sim \sum_{l=1}^L\lambda_l\mathcal{N}(\bfmu_l,\bfI_d),\label{notation_GMM}
\end{equation}
where $\lambda_l\in[0,1]$ with $\sum_l\lambda_l=1$, and $\mathcal{N}$ denotes the multi-variate Gaussian distribution with mean  $\bfmu_l\in \R^{d}$, and covariance $\bfI_d$ for all $l\in [L]$. Let $\bfM=(\bfmu_1,\bfmu_2,\cdots,\bfmu_L)$ and $\boldsymbol{\lambda}=(\lambda_1,\lambda_2,\cdots,\lambda_L)$. 
The teacher model in this paper is a fully connected neural network consisting of an input layer, a hidden layer, followed by a pooling layer. The number of neurons in the hidden layer is denoted as $K$. All neurons are equipped with Sigmoid activation functions\footnote{The results can be generalized to any even  activation  function $\phi$  with bounded  $\phi$, $\phi'$ and $\phi''$. Examples include $\tanh$ and $\text{erf}$.} $\phi(x)=\frac{1}{1+\exp(-x)}$. For any input $\bfx \in \mathcal{X}$, the output of the teacher model is denoted as 
\begin{equation} \label{cla_model}
H(\bfW^*;\bfx):=\frac{1}{K}\sum_{j=1}^K\phi({\bfw^*_j}^\top\bfx),
\end{equation}
where $\bfW^*=[\bfw^*_1,...,\bfw^*_K]\in \R^{d\times K}$ is an unknown fixed weight matrix, and $\bfw^*_j \in \R^{d}$  is the weight of the $j$-th neuron in the hidden layer. The corresponding output label $y$  satisfies
\begin{equation}
    \mathbb{P}(y=1|\bfx)=H(\bfW^*;\bfx).
\end{equation}
The training process is over a student neural network with the same architecture as the teacher model, and the trainable parameters are denoted as $\bfW\in \R^{d\times K}$. 
Given $n$ pairs of training samples $\{\bfx_i,y_i\}_{i=1}^n$ from $(\mathcal{X},\mathcal{Y})$, the empirical risk function is 
\begin{equation}\label{empirical}
f_n(\bfW)=\frac{1}{n}\sum_{i=1}^n \ell(\bfW;\bfx_i,y_i),
\end{equation}
and $\ell(\bfW;\cdot,\cdot)$ is the cross-entropy loss function as
\begin{equation}\label{cross-entropy}
\begin{aligned}
\ell(\bfW;\bfx,y)
=&-y\cdot\log(H(\bfW;\bfx))\\
&-(1-y)\cdot\log(1-H(\bfW;\bfx)).
\end{aligned}
\end{equation}
The neural network training problem is to minimize the following non-convex objective function:
\begin{equation}\label{eqn:problem} 
\min_{\bfW \in \R^{d\times K}}: \quad  f_n(\bfW).    
\end{equation}
$\bfW^*$ may not be a global optimal solution to \eqref{eqn:problem} because $y$ is the quantization of $H(\bfW^*;\bfx)$. However, $\bfW^*$ minimizes the expectation of \eqref{eqn:problem} over $(\mathcal{X},\mathcal{Y})$.
Note that for any permutation matrix $\bfP\in\mathbb{R}^{K\times K}$, we have  $H(\bfW;\bfx)=H(\bfW \bfP;\bfx)$, and $f_n(\bfW \bfP)=f_n(\bfW)$. Hence, the estimation is considered successful if one finds weights $\bfW$ close to any column permutation of $\bfW^*$. 

==> CISS_mixed_Gaussian (1)/simulation.tex <==
\section{Simulation}

Here we present our results for numerical experiments. All simulations are implemented in MATLAB 2021b on a workstation with 3.40GHz Intel Core i7. The weights of the teacher model $\bfW^*\in \R^{d\times K}$ are randomly generated such that each entry of $\bfW^*$ belongs to $\mathcal{N}(0,1)$. The corresponding training samples $\{\bfx_i, y_i\}_{i=1}^n$ are randomly selected following (\ref{notation_GMM}) and  (\ref{cla_model}) with the generated weights $\bfW^*$.  

\subsection{Sample complexity}
We first show how the number of required samples is related to the dimension of data. The parameters of input distribution are selected as $L=2$, $\lambda_1=\lambda_2=\frac{1}{2}$, $\bfmu_1=0.5*\boldsymbol{1}$ and $\bfmu_2=-\bfmu_1$. The number of neurons in the hidden layer is set as $3$. For a given $\bfW^*$, we initialize the starting point $M$ times randomly and denote $\widehat{\bfW}_n^{(m)}$ as the output of Algorithm \ref{gd} with the $m$-th initialization, and $M=20$. 
% The average estimation error $e_{\bfW^*}=\sqrt{\sum_{m=1}^M||\widehat{\bfW}_n^{(m)}-\bar{\bfW}_n||^2/M}$, where $\bar{\bfW}_n$ is the mean of $(\widehat{\bfW}_n^{(1)},\cdots, \widehat{\bfW}_n^{(L)})$. 
An experiment is viewed as a success if the average estimation error $e_{\bfW^*}$ is less than $10^{-3}$, where $e_{\bfW^*}$ is the standard deviation of $(\widehat{\bfW}_n^{(1)},\cdots, \widehat{\bfW}_n^{(L)})$.
  
In Fig.~\ref{fig:ntod},  we increase the feature dimension $d$ from 12 to 50 by 2 and vary the number of samples $n$ from $2\times 10^3$ to $3\times 10^4$. We test $20$ independent experiments for each pair of $d$ and $n$ and then show the average success rate using grey blocks, where black ones mean rate 0 and white ones mean rate 1. In Fig.~\ref{fig:ntod}, the boundary line of black and white parts is almost straight, indicating an approximate linearity between $n$ and $d$, which verifies our result in \eqref{final_sp}.
 \begin{figure}
\centering
\includegraphics[width=0.7\linewidth,height=0.5\linewidth]{Figure/sample_dimension.pdf}
\caption{The sample complexity against the feature dimension $d$}
\label{fig:ntod}

\end{figure}


We then study the impact on the sample complexity when the mean value in the Gaussian mixture model changes. Set $d=10$, $\lambda_1=0.4$, $\lambda_2=0.6$, $\bfmu_1=\mu \cdot\boldsymbol{1}$, $\bfmu_2=\boldsymbol{0}$. Fig.~\ref{figure: spmu} shows that when the mean increases from $0$ to $2$, the sample complexity increases, matching our theoretical analyses in Section \ref{sec: theory}. 
 \begin{figure}
\centering
\includegraphics[width=0.75\linewidth]{Figure/sample_mean.pdf}
\caption{The sample complexity when one mean changes}
\label{figure: spmu}

\end{figure}


\subsection{Convergence analysis}
We next fix $d=5$ and evaluate the convergence rate of Algorithm \ref{gd}. 
We set $n=1\times 10^4$, $\lambda_1=\lambda_2=0.5$, $\bfmu_1=-\bfmu_2=C\cdot\boldsymbol{1}$ for a positive $C$. We vary $C$ and let $\tilde{\mu}=\max_{l}\|\tilde{\bfmu_l}\|_\infty$. Recall the relative error is defined as $\|\bfW_t-\widehat{\bfW}_n\|_F$ in \eqref{linear convergence}. Fig.~\ref{figure: convergence_musigma} shows the linear convergence of Algorithm \ref{gd} for different $\tilde{\mu}$ and the impact of $\|\tilde{\bfmu}_l\|_\infty$. As predicted in Theorem \ref{thm1},  when $\tilde{\mu}$ increases, gradient descent converges slower.
 
 
 \begin{figure}
\centering
\includegraphics[width=0.7\linewidth,height=0.4\linewidth]{Figure/err_mu.pdf}
\caption{The convergence rate with different $\tilde{\mu}$}
\label{figure: convergence_musigma}

\end{figure}

==> CISS_mixed_Gaussian (1)/theorem.tex <==
\section{Theoretical results}\label{sec: theory}
% \subsection{Informal Theoretical Findings}
% The major insights of the major theorems as follows.
 



% \subsection{Formal Theorems}
Theorem 1 indicates that with sufficient number of samples as in \eqref{final_sp}, the iterates returned by proposed Algorithm \ref{gd} converge linearly to a critical point $\widehat{\bfW}_n$ near a permutation of the ground truth, denoted as $\bfW^*\bfP^*$. The distance between $\widehat{\bfW}_n$ and $\bfW^*\bfP^*$ are upper bounded as a function of the number of samples in \eqref{eqn:converge}. Additionally, the required number of samples depends on $\mathcal{\bfB}$, which is a function of input distributions in \eqref{notation_GMM}. 
\begin{thm}\label{thm1}
% Consider the binary classification problem with one-hidden-layer fully connected neural network as in (\ref{cla_model}). 
% Suppose  Assumption \ref{assumption1} holds, then there exist 
Given the samples from $(\mathcal{X},\mathcal{Y})$ 
with size $n$ satisfying
\begin{equation}
%\begin{aligned}
n \geq n_{\textrm{sc}}:=poly(\epsilon_0^{-1}, \kappa, K) \mathcal{B}(\boldsymbol{\lambda},\bfM) d\log^2{d}
  \label{final_sp}
%\end{aligned}
\end{equation}
for some $\epsilon_0\in(0,\frac{1}{4})$ and positive value functions $\mathcal{B}(\boldsymbol{\lambda},\bfM)$ and $q(\boldsymbol{\lambda},\bfM)$, with probability at least $1-d^{-10}$,
the iterates $\{\bfW_t\}_{t=1}^T$ returned by Algorithm \ref{gd} with step size $\eta_0=O\Big( \big(\sum_{l=1}^L\lambda_l(\|\tilde{\bfmu}_l\|_\infty+1)^2\big)^{-1}\Big)$  converge  linearly to a critical point $\widehat{\bfW}_n$ with the rate of convergence $v=1-K^{-2}q(\boldsymbol{\lambda},\bfM)$, i.e.,   
\begin{equation}
\begin{aligned}
 ||\bfW_t-\widehat{\bfW}_n||_F 
\leq  v^t||\bfW_0-\widehat{\bfW}_n||_F.
\label{linear convergence}
\end{aligned}
\end{equation}
Moreover, there exists a permutation matrix $\bfP^*$ such that the distance between $\bfW^*\bfP^*$ and $\widehat{\bfW}_n$ is bounded by
\begin{equation}\label{eqn:converge}
 ||\widehat{\bfW}_n-\bfW^*\bfP^*||_F \leq O\Big( K^{\frac{5}{2}}\cdot\sqrt{d\log{n}/n}\Big).
\end{equation}
\end{thm}
\textbf{Remark 1:} From \eqref{final_sp}, the required number of samples for successful estimation is a linear function of the input feature dimension $d$ and $\mathcal{B}(\boldsymbol{\lambda}, \bfM)$, where $\mathcal{B}$ is a function of the input distribution parameters. Note that the degree of freedom of $\bfW^*$ is $dK$, the sample complexity in \eqref{final_sp} is nearly order-wise optimal in terms of $d$. In addition, $\mathcal{B}(\boldsymbol{\lambda}, \bfM)$ is an increasing function of any entry of $\bfM$ (from Corollary 1 below), indicating that the sample complexity increases as the mean of any Gaussian component increases.

\textbf{Remark 2:} From \eqref{linear convergence}, the distance between the convergent point $\widehat{\bfW}_n$  and the ground truth $\bfW^*\bfP^*$ is in the order of $\sqrt{d\log n/n}$. When the number of samples increases, the convergent point moves closer to the ground truth, implying a smaller generalization error.
 
\textbf{Remark 3:} From \eqref{eqn:converge}, we can see that the iterations converge to $\widehat{\bfW}_n$ linearly, and the rate of convergence is $1-K^{-2}q(\boldsymbol{\lambda},\bfM)$, denoted as $\nu$. When the number of neurons decreases or the input distribution changes such that $q$ increases, the rate of convergence decreases, indicating a faster convergence. 


% The sample complexity for estimation is  $\Theta(d\log^2{d})$, where $d$ is the feature dimension. Our bound is  almost order-wise optimal with respect to $d$ because the degree of freedom is $dK$. The additional multiplier of $\log^2{d}$ comes from the concentration bound in the proof technique. Note that we focus on the dependence of the sample complexity on the feature dimension $d$ and treat the network width $K$ as constant. Our result is in the same order as the sample complexity for  the standard Gaussian input in \cite{FCL20} and \cite{ZSJB17}, indicating that our technique can handle input from the Gaussian mixture model without increasing the order of the sample complexity. 


% \textbf{Remark 3:} 
% \textbf{3. Impact of  the mean}:
% If everything else is fixed, and at least 
% one entry of a mean $\mu_{l(i)}$ (the $i$th entry of $\bfmu_l$) of the Gaussian mixture model increases from 0 to infinity (in terms of the absolute value),  the sample complexity increases to infinity from a constant and the convergence slows down. The explanation is that when the absolute value of some mean increases, some training samples have a significantly large magnitude such that the sigmoid function saturates. The gradient of these samples is close to zero, so they are not informative for estimating $\bfW^*$. Therefore, the required samples complexity for estimation needs to increase,  and the gradient descent algorithm slows down. 


Corollary \ref{prop: diag_Cor} states the impact of the distribution parameters $\lambda$ and $\bfM$.
% $\mathcal{B}(\boldsymbol{\lambda},\bfM)$ and $q(\boldsymbol{\lambda},\bfM)$
% on the sample complexity $n_{\textrm{sc}}$ and the convergence rate $v$. 
Specifically, when the mean vectors $\{\bfmu_l\}_{l=1}^M$ in \eqref{notation_GMM} increases, the sample complexity $n_{\textrm{sc}}$ increases as $\mathcal{B}(\boldsymbol{\lambda},\bfM)$ increases, and the convergence rate $v$ increases as $q(\boldsymbol{\lambda},\bfM)$ decreases. Suppose some entry of $\bfmu_l$ go to infinity, $n_{\textrm{sc}}$ will go to infinity, and $\nu$ will converge to $1$.
\begin{corollary}\label{prop: diag_Cor} Recall $\bfM=(\bfmu_1,\cdots,\bfmu_L)$. Let $|\bfmu_{l(i)}|$  be the $i$-th entry of $\bfmu_l$,
\begin{enumerate}
    \item $\mathcal{B}(\boldsymbol{\lambda}, \bfM)$ is an increasing function of $|\bfmu_{l(i)}|$.
    \item $q(\boldsymbol{\lambda},\bfM)$ is a decreasing function of $|\bfmu_{l(i)}|$.
\end{enumerate} 
\end{corollary}



% Theorem \ref{thm1} shows that the empirical risk function in (\ref{empirical}) is strongly convex in a region near $\bfW^*\bfP$ for some permutation matrix $\bfP$. Subroutine 1 initializes one point in this convex region, and then the gradient descent finds a critical point in that region. We next summarize 
\iffalse
\subsection{Sketchy of the Proof}
% \textbf{Technical contributions.}
Following the line of works like \cite{ZSJB17, FCL20}, our proof of Theorem \ref{thm1} applies a two-stage approach: the convex analysis around a permutation of $\bfW^*$, and a good initialization lying in a convex region. The new technical contributions for our analysis are as follows. 

\textbf{(1) Local convexity.} To show the strong local convexity around a permutation of the ground truth, we need the lower bound of the Hessian of the population risk to be positive. However, the existing analysis in \cite{ZSJB17, FCL20} does not extend to the Gaussian mixture model. New tools are developed such that we can explicitly quantify the impact of the parameters of the input distribution on the landscapes of risk functions.  

\textbf{(2) Sample complexity.} The existing matrix concentration inequalities in \cite{ZSJB17, FCL20} leads to a loose sample complexity bound as $O(d^3)$ for non-zero mean Gaussian distributions (a sub-problem for Gaussian mixture models). We develop new concentration bounds to tighten the sample complexity in the order of $d\log^2 d$ for Gaussian mixture models.   

\textbf{(3) Tensor constructions.} The existing tensor initialization in \cite{ZSJB17, FCL20} only holds for Gaussian inputs. In this paper, new tensors are designed as in \eqref{eqn:mj}, and new concentration theorems are developed to bound the errors between the estimated tensors from a finite number of data and their theoretical values.
\fi

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************

